Prediction-assistant Frame Super-Resolution for Video Streaming

Video frame transmission delay is critical in real-time applications such as online video gaming, live show, etc. The receiving deadline of a new frame must catch up with the frame rendering time. Otherwise, the system will buffer a while, and the user will encounter a frozen screen, resulting in unsatisfactory user experiences. An effective approach is to transmit frames in lower-quality under poor bandwidth conditions, such as using scalable video coding. In this paper, we propose to enhance video quality using lossy frames in two situations. First, when current frames are too late to receive before rendering deadline (i.e., lost), we propose to use previously received high-resolution images to predict the future frames. Second, when the quality of the currently received frames is low~(i.e., lossy), we propose to use previously received high-resolution frames to enhance the low-quality current ones. For the first case, we propose a small yet effective video frame prediction network. For the second case, we improve the video prediction network to a video enhancement network to associate current frames as well as previous frames to restore high-quality images. Extensive experimental results demonstrate that our method performs favorably against state-of-the-art algorithms in the lossy video streaming environment.

==> PID253/ablation_figures/acc_scale.tex <==
\begin{figure}[t]
	\footnotesize
    % \scriptsize

	\centering
% 	\renewcommand{\tabcolsep}{1.0pt} % adjust horizontal space
% 	\renewcommand{\arraystretch}{1.0} % adjust vertical space
% 	\begin{tabular}{c}
	\includegraphics[width= 0.47\textwidth]{ablation_figures/acc_scale.png}
	
% \end{tabular}
 	\vspace{-5pt}
	\caption{
		\textbf{Analysis of the accuracy of optical flow estimation considering scaling factor on the Sintel~\cite{sintel} dataset.}
		%
		%
		We estimate the optical flow $\mathbf{E}(\mathbf{I}_0;~\texttt{bic}(\mathbf{I}_t^{\downarrow s}))$, where $\mathbf{E}$ refers to PWC-Net~\cite{sun2018pwc}, $\texttt{bic}(\mathbf{I}_1^{\downarrow s})$ is the bicubic interpolated frame.
	}
 	\vspace{-10pt}
	\label{fig:acc_scale} 
\end{figure}



==> PID253/ablation_figures/acc_scale_vis.tex <==
\begin{figure*}[t]
	\footnotesize
	%\tiny
	%\scriptsize
	\centering
	\renewcommand{\tabcolsep}{2.0pt} % adjust horizontal space
	\renewcommand{\arraystretch}{1.2} % adjust vertical space
	\begin{tabular}{cccccc}
                % \multicolumn{2}{c}{\includegraphics[width=0.5\linewidth, height=0.2\linewidth]{preface-figure/blurry_overlap/blurry.png}} &
                \includegraphics[width=0.16\linewidth]{ablation_figures/flow_prop_figure/f_10_11_s.png} &
                \includegraphics[width=0.16\linewidth]{ablation_figures/flow_prop_figure/f_ested_x4_s.png} &
                 \includegraphics[width=0.16\linewidth]{ablation_figures/flow_prop_figure/f_ested_x8_s.png} &
				  \includegraphics[width=0.16\linewidth]{ablation_figures/flow_prop_figure/f_prop_s.png} &
			 \includegraphics[width=0.16\linewidth]{ablation_figures/flow_prop_figure/f_warp_s.png} &
			 \includegraphics[width=0.16\linewidth]{ablation_figures/flow_prop_figure/f_ested_x1_s.png} 
			    \\
			    (a) overlayed inputs &
				(b) estimated ($s=4$) &
				(c) estimated ($s=8$) &
				(d) propagated &
				(e) warped &
				(f) fused 
				\\
	\end{tabular}
	\vspace{-5pt}
	\caption{
        \textbf{Visualizations of optical flow outputs of prediction, propagation and estimation schemes on the Sintel dataset~\cite{sintel}.}
        %
	}
	\label{fig:flow_acc_scale} %% label for entire figure
	\vspace{-5pt}
\end{figure*}

==> PID253/ablation_tables/ablation_table.tex <==
\begin{table}[t]
  \caption{
     \textbf{Ablation experiments to quantitatively analyze the effect of the different components of our model for next frame super-resolution.}
  }
%   \vspace{-1mm}
  \label{tab:abla_component}
  \footnotesize
% \scriptsize

  \renewcommand{\tabcolsep}{1.6pt} % adjust horizontal space
  \renewcommand{\arraystretch}{1.2} % adjust vertical space
  \newcommand{\quantTit}[1]{\multicolumn{3}{c}{\scriptsize #1}}
    \newcommand{\quantSec}[1]{\scriptsize #1}
    \newcommand{\quantInd}[1]{\scriptsize #1}
    \newcommand{\quantVal}[1]{\scalebox{0.83}[1.0]{$ #1 $}}
    \newcommand{\quantBes}[1]{\scalebox{0.83}[1.0]{$\uline{ #1 }$}}
    
  \centering
  \begin{tabular}{lcccccccc}
    \toprule
    

    \multirow{4}{*}[-0.28em]{Method}   
     & \multicolumn{4}{c}{Vimeo90K~\cite{xue2019video}}
     & \multicolumn{4}{c}{Middlebury~\cite{baker2011database}}

     
     \\
        \cmidrule(lr){2-5}
        \cmidrule(lr){6-9}

     & \multicolumn{2}{c}{ 4 $\times$}
     & \multicolumn{2}{c}{ 8 $\times$} 
 
     & \multicolumn{2}{c}{ 4 $\times$}
     & \multicolumn{2}{c}{ 8 $\times$} 
     


     \\
    
        \cmidrule(lr){2-3}
        \cmidrule(lr){4-5}
        \cmidrule(lr){6-7}
        \cmidrule(lr){8-9}
 
    
    &  \quantSec{PSNR} & \quantSec{SSIM}  & \quantSec{PSNR} & \quantSec{SSIM}  
     & \quantSec{PSNR} & \quantSec{SSIM}  & \quantSec{PSNR} & \quantSec{SSIM} 

    \\
    
    \midrule
        Bicubic 
              
              & \quantVal{29.77} &  \quantVal{0.903}
              & \quantVal{25.79} &  \quantVal{0.824}
              
              & \quantVal{27.71}  & \quantVal{0.858}
              & \quantVal{23.82}  & \quantVal{0.763}
    \\
 
             
        \midrule
        
         PA - FlowNet2-S
              
              & \quantVal{39.79} & \quantVal{0.974}
              & \quantVal{37.84} & \quantVal{0.961}
              
              & \quantVal{35.04} & \quantVal{0.948}
              & \quantVal{\second{32.16}} & \quantVal{\second{0.936}}
              
              \\
        
        PA - PWC-Net
              
              & \quantVal{\second{41.01}} & \quantVal{\second{0.978}}
              & \quantVal{\second{37.98}} & \quantVal{\second{0.964}}
              
              & \quantVal{\second{35.18}} & \quantVal{\second{0.952}}
              & \quantVal{{32.15}} & \quantVal{\second{0.936}}
              
              \\
        
        PA - PWC-Net-ft
              
              & \quantVal{\first{41.72}} & \quantVal{\first{0.989}}
              & \quantVal{\first{38.81}} & \quantVal{\first{0.982}}
              
              & \quantVal{\first{36.40}} & \quantVal{\first{0.967}}
              & \quantVal{\first{33.66}} & \quantVal{\first{0.948}}
              
              \\
        
        \midrule
        
        PA - \textit{only f-estimation}
              
              & \quantVal{40.02} & \quantVal{0.968}
              & \quantVal{36.71} & \quantVal{0.956}
              
              & \quantVal{35.45} & \quantVal{0.947}
              & \quantVal{32.84} & \quantVal{0.926}
              
              \\
              
              
               PA - \textit{w/ f-propagation}
              
              & \quantVal{40.45} & \quantVal{0.970}
              & \quantVal{37.11} & \quantVal{0.962}
              
              
              & \quantVal{36.14} & \quantVal{0.959}
              & \quantVal{33.22} & \quantVal{0.932}

              \\
        
                PA -\textit{ w/ f-warping}
              & \quantVal{\second{40.46}} & \quantVal{\second{0.970}}
              & \quantVal{\second{37.41}} & \quantVal{\second{0.969}}
              
              
              & \quantVal{\second{36.22}} & \quantVal{\second{0.960}}
              & \quantVal{\second{33.43}} & \quantVal{\second{0.935}}
   
              \\
             
        PA
              
              & \quantVal{\first{41.72}} & \quantVal{\first{0.989}}
              & \quantVal{\first{38.81}} & \quantVal{\first{0.982}}
              
              & \quantVal{\first{36.40}} & \quantVal{\first{0.967}}
              & \quantVal{\first{33.66}} & \quantVal{\first{0.948}}
              
              \\
              
        \bottomrule


  \end{tabular}
    \vspace{-5pt}  
\end{table}




==> PID253/ablation_tables/flow_prop.tex <==
\begin{table}[t]
  \caption{
     \textbf{Analysis of flow propagation and estimation using the Sintel~\cite{sintel} dataset.}
     %
     For frame prediction, we take three previous frames $\mathbf{I}_{-2}, \mathbf{I}_{-1}, \mathbf{I}_{0}$ as inputs to \underline{propagate} or warp the optical flow of the next frame, denoted by \underline{$\mathbf{\tilde{F}}_{0 \rightarrow 1}$}, $\mathbf{\hat{F}}_{0 \rightarrow 1}$.
     %
     For frame estimation, we use the current frame $\mathbf{I}_0$ and the next frame $\mathbf{I}_1$ of full-resolution to estimate optical flow $\mathbf{\bar{F}}_{0 \rightarrow 1}$.
     %
     We compare the output flow with the ground truth at every pixel using end-point-error (EPE).
     %
     The numbers in \first{red} and \second{blue} represent the best and second-best results.
  }
%   \vspace{-5pt}
  \label{tab:flow_prop}
  \footnotesize
  
  \renewcommand{\tabcolsep}{1.5pt} % adjust horizontal space
  \renewcommand{\arraystretch}{1.2} % adjust vertical space
\newcommand{\quantTit}[1]{\multicolumn{3}{c}{\scriptsize #1}}
    \newcommand{\quantSec}[1]{\scriptsize #1}
    \newcommand{\quantInd}[1]{\scriptsize #1}
    \newcommand{\quantVal}[1]{\scalebox{0.83}[1.0]{$ #1 $}}
    \newcommand{\quantBes}[1]{\scalebox{0.83}[1.0]{$\uline{ #1 }$}}
  \centering
  \begin{tabular}{lccc cccc c}
    \toprule
    
    % \multirow{2}{*}[-0.28em]{Method}   
    % %  & Runtime 
    % % & Parameters 
    %  &  \multicolumn{2}{c}{111}
    %   & \multicolumn{2}{c}{YouTube240} \\
    
    % %  \cmidrule(l{2pt}r{1pt}){2-3}
    % % \cmidrule(l{2pt}r{1pt}){4-5} 
    % \cmidrule(lr){2-3}
    % \cmidrule(lr){4-5}
    
    % % %\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){a-b}
    % & PSNR & SSIM  &PSNR & SSIM \\
    
    clips &  \quantSec{\text{market2}} & 
    \quantSec{\text{alley2}} & 
    \quantSec{\text{sleeping1}} & 
    \quantSec{\text{ambush6}} & 
    \quantSec{\text{alley1}} & 
    \quantSec{\text{temple2}} & 
    \quantSec{\text{cave4}}
    \\
    
    
    \midrule
    
    \multicolumn{8}{c}{ \quantSec{ Using FlowNet2-S~\cite{IMKDB17}}} 
    
    \\
    
    \midrule
        
        Propagation $\mathbf{\tilde{F}}_{0 \rightarrow 1}$ &
            
            \quantVal{2.586} & %market\_2
            \quantVal{1.653} & %alley\_2  
            \quantVal{0.919} & %sleeping\_1
            \quantVal{27.65} & %ambush\_6 
            \quantVal{1.684} & %alley\_1 
            \quantVal{6.937} & %temple\_2 
            \quantVal{9.938} % cave\_4
            
        \\
        Warping~~~~~~ $\mathbf{\hat{F}}_{0 \rightarrow 1}$ &
          
            \quantVal{\second{1.798}} & %market\_2
            \quantVal{\second{1.001}} & %alley\_2  
            \quantVal{\second{0.536}} & %sleeping\_1
            \quantVal{\second{25.46}} & %ambush\_6 
            \quantVal{\second{1.028}} & %alley\_1 
            \quantVal{\second{5.353}} & %temple\_2 
            \quantVal{\second{8.052}} % cave\_4
        \\
        
        Estimation~~ $\mathbf{\bar{F}}_{0 \rightarrow 1}$ &
          
            \quantVal{\first{1.306}} & %market\_2
            \quantVal{\first{0.770}} & %alley\_2  
            \quantVal{\first{0.528}} & %sleeping\_1
            \quantVal{\first{9.198}} & %ambush\_6 
            \quantVal{\first{0.818}} &%alley\_1 
            \quantVal{\first{3.059}} & %temple\_2 
            \quantVal{\first{5.227}} % cave\_4
            
        \\
    
          
        
        \midrule
        
        \multicolumn{8}{c}{ \quantSec{Using PWC-Net~\cite{sun2018pwc} }} 
        
        \\
        
        \midrule 
        
        Propagation $\mathbf{\tilde{F}}_{0 \rightarrow 1}$ &
          
            \quantVal{1.442} & %market\_2
            \quantVal{\second{0.561}} & %alley\_2  
            \quantVal{\second{0.287}} & %sleeping\_1
            \quantVal{\second{24.33}} & %ambush\_6 
            \quantVal{\second{0.587}} & %alley\_1 
            \quantVal{6.990} & %temple\_2 
            \quantVal{9.393} % cave\_4
           
        
        \\
        
        Warping~~~~~~ $\mathbf{\hat{F}}_{0 \rightarrow 1}$ &
             
            \quantVal{\second{1.297}}  & %market\_2
            \quantVal{0.757} & %alley\_2  
            \quantVal{0.139} & %sleeping\_1
            \quantVal{26.05}  & %ambush\_6 
            \quantVal{0.589} & %alley\_1 
            \quantVal{\second{4.171}} & %temple\_2 
            \quantVal{\second{7.643}} % cave\_4
        \\
        
        Estimation~~ $\mathbf{\bar{F}}_{0 \rightarrow 1}$ &

             

            \quantVal{\first{0.606}} & %market\_2
            \quantVal{\first{0.279}} & %alley\_2  
            \quantVal{\first{0.126}} & %sleeping\_1
            \quantVal{\first{5.320}} & %ambush\_6 
            \quantVal{\first{0.271}} & %alley\_1 
            \quantVal{\first{1.863}} &%temple\_2 
            \quantVal{\first{3.260}} % cave\_4
            
        \\
        
        % \midrule
        
        % Predict Fusion $\mathbb{{\hat{F}}}_{0 \rightarrow 1}$ &
        %      PWC-Net~\cite{sun2018pwc} &
            
        %     %market\_2
        %     %alley\_2  %sleeping\_1
        %     %ambush\_6 
        %     %alley\_1 
        %     %temple\_2 
        %     % cave\_4 
        %     \\
            
        % Estimate Fusion $\mathbb{{\bar{F}}}_{0 \rightarrow 1}$ &
        %      PWC-Net~\cite{sun2018pwc} &
            
        %     %market\_2
        %     %alley\_2  %sleeping\_1
        %     %ambush\_6 
        %     %alley\_1 
        %     %temple\_2 
        %     % cave\_4 
        %     \\
        
        
       
       
       
  
        \bottomrule


  \end{tabular}
    \vspace{-5pt}  
\end{table}



==> PID253/compare_figures/multiple_gap_comparison.tex <==
\begin{figure}[t]
	\footnotesize
    % \scriptsize

	\centering
% 	\renewcommand{\tabcolsep}{1.0pt} % adjust horizontal space
% 	\renewcommand{\arraystretch}{1.0} % adjust vertical space
% 	\begin{tabular}{c}
	\includegraphics[width= 0.47\textwidth]{compare_figures/multiple_gap_comparison.png}
	
% \end{tabular}
 	\vspace{-5pt}
	\caption{
		\textbf{Comparisons of video super-resolution using different frame gaps on the Vimeo90K evaluation dataset~\cite{xue2019video}.}
		%
		%
		Our model is trained using a frame gap equals to one, and we test the model using frames with multiple gaps.
	}
 	\vspace{-10pt}
	\label{fig:multiple_gap} 
\end{figure}



==> PID253/compare_figures/vis_compare_middlebury.tex <==
\begin{figure*}[!th]
	\footnotesize
% 	\tiny 
	\scriptsize        
	\centering
	\renewcommand{\tabcolsep}{0.25pt} % adjust horizontal space
	\renewcommand{\arraystretch}{1.0} % adjust vertical space
	\begin{tabular}{ccccc ccccc}


% \multirow{3}{*}[10.10em]{\includegraphics[width=0.22\linewidth]{compare_figures/middlebury/gt_s.png}} &

\includegraphics[width=0.099\linewidth]{compare_figures/middlebury1/gt_s.png}&
\includegraphics[width=0.099\linewidth]{compare_figures/middlebury1/bic.png}&
\includegraphics[width=0.099\linewidth]{compare_figures/middlebury1/edsr.png}&
\includegraphics[width=0.099\linewidth]{compare_figures/middlebury1/toflow.png}&
\includegraphics[width=0.099\linewidth]{compare_figures/middlebury1/duf.png} &

\includegraphics[width=0.099\linewidth]{compare_figures/middlebury1/edvr.png}  &
\includegraphics[width=0.099\linewidth]{compare_figures/middlebury1/crossnet.png}&
\includegraphics[width=0.099\linewidth]{compare_figures/middlebury1/awnet.png} &
\includegraphics[width=0.099\linewidth]{compare_figures/middlebury1/ours.png} &
\includegraphics[width=0.099\linewidth]{compare_figures/middlebury1/gt.png}
\\

\includegraphics[width=0.099\linewidth]{compare_figures/middlebury2/gt_s.png}&
\includegraphics[width=0.099\linewidth]{compare_figures/middlebury2/bic.png}&
\includegraphics[width=0.099\linewidth]{compare_figures/middlebury2/edsr.png}&
\includegraphics[width=0.099\linewidth]{compare_figures/middlebury2/toflow.png}&
\includegraphics[width=0.099\linewidth]{compare_figures/middlebury2/duf.png} &

\includegraphics[width=0.099\linewidth]{compare_figures/middlebury2/edvr.png}  &
\includegraphics[width=0.099\linewidth]{compare_figures/middlebury2/crossnet.png}&
\includegraphics[width=0.099\linewidth]{compare_figures/middlebury2/awnet.png} &
\includegraphics[width=0.099\linewidth]{compare_figures/middlebury2/ours.png} &
\includegraphics[width=0.099\linewidth]{compare_figures/middlebury2/gt.png}
\\


GT & 
Bicubic &
EDSR &
TOFlow &
DUF &
EDVR &
CrossNet &
AWnet &
Ours &
GT 

\\



\end{tabular}
	\vspace{-5pt}
	\caption{
       \textbf{Visual comparisons on the Middlebury set~\cite{baker2011database}.}
	   %
	}
	\label{fig:compare_middlebury} %% label for entire figure
	\vspace{-10pt}
\end{figure*}


==> PID253/compare_figures/vis_compare_reds.tex <==
\begin{figure*}[!th]
	\footnotesize
% 	\tiny 
	\scriptsize        
	\centering
	\renewcommand{\tabcolsep}{0.12pt} % adjust horizontal space
	\renewcommand{\arraystretch}{1.0} % adjust vertical space
	\begin{tabular}{ccccc ccccc}


% \multirow{3}{*}[10.10em]{\includegraphics[width=0.22\linewidth]{compare_figures/middlebury/gt_s.png}} &

\includegraphics[width=0.099\linewidth]{compare_figures/reds/gt_s.png}&
\includegraphics[width=0.099\linewidth]{compare_figures/reds/bic.png}&
\includegraphics[width=0.099\linewidth]{compare_figures/reds/edsr.png}&
\includegraphics[width=0.099\linewidth]{compare_figures/reds/toflow.png}&
\includegraphics[width=0.099\linewidth]{compare_figures/reds/duf.png} &

\includegraphics[width=0.099\linewidth]{compare_figures/reds/edvr.png}  &
\includegraphics[width=0.099\linewidth]{compare_figures/reds/crossnet.png}&
\includegraphics[width=0.099\linewidth]{compare_figures/reds/awnet.png} &
\includegraphics[width=0.099\linewidth]{compare_figures/reds/ours.png} &
\includegraphics[width=0.099\linewidth]{compare_figures/reds/gt.png}
\\



GT & 
Bicubic &
EDSR &
TOFlow &
DUF &
EDVR &
CrossNet &
AWnet &
Ours &
GT 

\\



\end{tabular}
	\vspace{-5pt}
	\caption{
       \textbf{Visual comparisons on the REDS set~\cite{Nah_2019_CVPR_Workshops_SR}.}
	   %
	}
	\label{fig:compare_reds} %% label for entire figure
	\vspace{-10pt}
\end{figure*}


==> PID253/compare_figures/vis_compare_vid4.tex <==
\begin{figure*}[!th]
	\footnotesize
% 	\tiny 
	\scriptsize        
	\centering
	\renewcommand{\tabcolsep}{0.12pt} % adjust horizontal space
	\renewcommand{\arraystretch}{1.0} % adjust vertical space
	\begin{tabular}{ccccc ccccc}


% \multirow{3}{*}[10.10em]{\includegraphics[width=0.22\linewidth]{compare_figures/middlebury/gt_s.png}} &

\includegraphics[width=0.099\linewidth]{compare_figures/vid4/gt_s.png}&
\includegraphics[width=0.099\linewidth]{compare_figures/vid4/bic.png}&
\includegraphics[width=0.099\linewidth]{compare_figures/vid4/edsr.png}&
\includegraphics[width=0.099\linewidth]{compare_figures/vid4/toflow.png}&
\includegraphics[width=0.099\linewidth]{compare_figures/vid4/duf.png} &

\includegraphics[width=0.099\linewidth]{compare_figures/vid4/edvr.png}  &
\includegraphics[width=0.099\linewidth]{compare_figures/vid4/crossnet.png}&
\includegraphics[width=0.099\linewidth]{compare_figures/vid4/awnet.png} &
\includegraphics[width=0.099\linewidth]{compare_figures/vid4/ours.png} &
\includegraphics[width=0.099\linewidth]{compare_figures/vid4/gt.png}
\\



GT & 
Bicubic &
EDSR &
TOFlow &
DUF &
EDVR &
CrossNet &
AWnet &
Ours &
GT 

\\



\end{tabular}
	\vspace{-5pt}
	\caption{
       \textbf{Visual comparisons on the Vid4 set~\cite{liu2013bayesian}.}
	   %
	}
	\label{fig:compare_vid4} %% label for entire figure
	\vspace{-10pt}
\end{figure*}


==> PID253/compare_figures/vis_compare_vimeo.tex <==
\begin{figure*}[!th]
	\footnotesize
% 	\tiny 
	\scriptsize        
	\centering
	\renewcommand{\tabcolsep}{0.20pt} % adjust horizontal space
	\renewcommand{\arraystretch}{1.0} % adjust vertical space
	\begin{tabular}{ccccc ccccc}


% \multirow{3}{*}[10.10em]{\includegraphics[width=0.22\linewidth]{compare_figures/middlebury/gt_s.png}} &

\includegraphics[width=0.099\linewidth]{compare_figures/vimeo1/gt_s.png}&
\includegraphics[width=0.099\linewidth]{compare_figures/vimeo1/bic.png}&
\includegraphics[width=0.099\linewidth]{compare_figures/vimeo1/edsr.png}&
\includegraphics[width=0.099\linewidth]{compare_figures/vimeo1/toflow.png}&
\includegraphics[width=0.099\linewidth]{compare_figures/vimeo1/duf.png} &

\includegraphics[width=0.099\linewidth]{compare_figures/vimeo1/edvr.png}  &
\includegraphics[width=0.099\linewidth]{compare_figures/vimeo1/crossnet.png}&
\includegraphics[width=0.099\linewidth]{compare_figures/vimeo1/awnet.png} &
\includegraphics[width=0.099\linewidth]{compare_figures/vimeo1/ours.png} &
\includegraphics[width=0.099\linewidth]{compare_figures/vimeo1/gt.png}
\\

\includegraphics[width=0.099\linewidth]{compare_figures/vimeo2/gt_s.png}&
\includegraphics[width=0.099\linewidth]{compare_figures/vimeo2/bic.png}&
\includegraphics[width=0.099\linewidth]{compare_figures/vimeo2/edsr.png}&
\includegraphics[width=0.099\linewidth]{compare_figures/vimeo2/toflow.png}&
\includegraphics[width=0.099\linewidth]{compare_figures/vimeo2/duf.png} &

\includegraphics[width=0.099\linewidth]{compare_figures/vimeo2/edvr.png}  &
\includegraphics[width=0.099\linewidth]{compare_figures/vimeo2/crossnet.png}&
\includegraphics[width=0.099\linewidth]{compare_figures/vimeo2/awnet.png} &
\includegraphics[width=0.099\linewidth]{compare_figures/vimeo2/ours.png} &
\includegraphics[width=0.099\linewidth]{compare_figures/vimeo2/gt.png}
\\


GT & 
Bicubic &
EDSR &
TOFlow &
DUF &
EDVR &
CrossNet &
AWnet &
Ours &
GT 

\\



\end{tabular}
	\vspace{-5pt}
	\caption{
       \textbf{Visual comparisons on the Vimeo90K set~\cite{xue2019video}.}
	   %
	}
	\label{fig:compare_vimeo} %% label for entire figure
	\vspace{-10pt}
\end{figure*}


==> PID253/compare_tables/compare_next_frame_sr.tex <==
\begin{table*}[t]
  \caption{
     \textbf{Quantitative comparisons of various state-of-the-art methods for next frame super-resolution.}
  }
%   \vspace{-5pt}
  \label{tab:compare_next_frame_sr}
  \footnotesize
% \scriptsize

  \renewcommand{\tabcolsep}{1.5pt} % adjust horizontal space
  \renewcommand{\arraystretch}{1.2} % adjust vertical space
  \newcommand{\quantTit}[1]{\multicolumn{3}{c}{\scriptsize #1}}
    \newcommand{\quantSec}[1]{\scriptsize #1}
    \newcommand{\quantInd}[1]{\scriptsize #1}
    \newcommand{\quantVal}[1]{\scalebox{0.83}[1.0]{$ #1 $}}
    \newcommand{\quantBes}[1]{\scalebox{0.83}[1.0]{$\uline{ #1 }$}}
    
  \centering
  \begin{tabular}{lccccccccccccccccccccc}
    \toprule
    

    
    \multirow{4}{*}[-0.28em]{Method}   
     &
     & \multicolumn{4}{c}{Vimeo90K~\cite{xue2019video}}
     & \multicolumn{4}{c}{Middlebury~\cite{baker2011database}}
      & \multicolumn{4}{c}{Vid4~\cite{liu2013bayesian}}
      & \multicolumn{4}{c}{REDS~\cite{Nah_2019_CVPR_Workshops_SR}}
        & \multicolumn{4}{c}{HD~\cite{bao2018memc}}
     
     \\
        \cmidrule(lr){3-6}
        \cmidrule(lr){7-10}
        \cmidrule(lr){11-14}
        \cmidrule(lr){15-18}
        \cmidrule(lr){19-22}
     &
     & \multicolumn{2}{c}{ 4 $\times$}
     & \multicolumn{2}{c}{ 8 $\times$} 
 
     & \multicolumn{2}{c}{ 4 $\times$}
     & \multicolumn{2}{c}{ 8 $\times$} 
     
     & \multicolumn{2}{c}{ 4 $\times$}
     & \multicolumn{2}{c}{ 8 $\times$} 
     
     & \multicolumn{2}{c}{ 4 $\times$}
     & \multicolumn{2}{c}{ 8 $\times$} 
     
     & \multicolumn{2}{c}{ 4 $\times$}
     & \multicolumn{2}{c}{ 8 $\times$} 

     \\
    
        \cmidrule(lr){3-4}
        \cmidrule(lr){5-6}
        \cmidrule(lr){7-8}
        \cmidrule(lr){9-10}
        \cmidrule(lr){11-12}
        \cmidrule(lr){13-14}
        \cmidrule(lr){15-16}
        \cmidrule(lr){17-18}
        \cmidrule(lr){19-20}
        \cmidrule(lr){21-22}
    
    & & \quantSec{PSNR} & \quantSec{SSIM}  & \quantSec{PSNR} & \quantSec{SSIM}  
     & \quantSec{PSNR} & \quantSec{SSIM}  & \quantSec{PSNR} & \quantSec{SSIM} 
     & \quantSec{PSNR} & \quantSec{SSIM}  & \quantSec{PSNR} & \quantSec{SSIM} 
     & \quantSec{PSNR} & \quantSec{SSIM}  & \quantSec{PSNR} & \quantSec{SSIM} 
     & \quantSec{PSNR} & \quantSec{SSIM}  & \quantSec{PSNR} & \quantSec{SSIM} 
    \\
    
    \midrule
        Bicubic 
              & \multirow{2}{*}{\quantSec{1~LR}}
              
              & \quantVal{29.77} &  \quantVal{0.903}
              & \quantVal{25.79} &  \quantVal{0.824}
              
              & \quantVal{27.71}  & \quantVal{0.858}
              & \quantVal{23.82}  & \quantVal{0.763}
              
              & \quantVal{22.37} & \quantVal{0.610}
              & \quantVal{19.82} & \quantVal{0.615}
              
              & \quantVal{26.29} & \quantVal{0.801}
              & \quantVal{23.48} & \quantVal{0.702}
              
              & \quantVal{32.98} & \quantVal{0.936}
              & \quantVal{28.06} & \quantVal{0.880}
              
              \\
        EDSR~\cite{Lim_2017_CVPR_Workshops}
              & 
              & \quantVal{33.11}  & \quantVal{0.941} 
              
              & \quantVal{28.20}  & \quantVal{0.870}
              
              & \quantVal{30.92} & \quantVal{0.905}
              & \quantVal{26.55} & \quantVal{0.813}
              
              & \quantVal{24.06} & \quantVal{0.818}
              & \quantVal{20.80}& \quantVal{0.678}
              
               
              & \quantVal{28.51} & \quantVal{0.857}
              & \quantVal{25.05} & \quantVal{0.754}
              
               
              & \quantVal{35.68}  & \quantVal{0.957}
              & \quantVal{30.61}  &\quantVal{0.909}
        
              \\
    \midrule          
              
      ToFlow-SR~\cite{xue2019video}
              & \multirow{3}{*}{\quantSec{7~LR}}
              & \quantVal{33.08} & \quantVal{0.942}
              & \quantVal{28.35} & \quantVal{0.882}
              
              & \quantVal{30.27} & \quantVal{0.897}
              & \quantVal{26.02} & \quantVal{0.801}
              
              & \quantVal{24.41} & \quantVal{0.743}
              & \quantVal{21.49} & \quantVal{0.712}
              
              & \quantVal{27.98}  & \quantVal{0.799}
              &  \quantVal{23.59} & \quantVal{0.725}
              
              & \quantVal{33.55} & \quantVal{0.929}
              & \quantVal{27.01} & \quantVal{0.856}
              
              \\
              
         DUF~\cite{jo2018deep}
              &
              & \quantVal{34.33} & \quantVal{0.922}
              & \quantVal{28.55} & \quantVal{0.901}
              
              
              & \quantVal{30.89} & \quantVal{0.915}
              & \quantVal{27.46} & \quantVal{0.828}
              
              & \quantVal{25.79} & \quantVal{0.814}
              & \quantVal{21.42} & \quantVal{0.714}  
              
              & \quantVal{28.63} & \quantVal{0.825}
              & \quantVal{24.57} & \quantVal{0.788}
              
              & \quantVal{34.15} & \quantVal{0.926}
              & \quantVal{28.45} & \quantVal{0.891}
              
              \\
    
              
        EDVR~\cite{wang2019edvr}
              &
              & \quantVal{35.79} & \quantVal{0.937}
              & \quantVal{29.93} & \quantVal{0.896}
              
              & \quantVal{31.91} & \quantVal{0.924}
              & \quantVal{27.53} & \quantVal{0.832}
              
              & \quantVal{25.83} & \quantVal{0.808}
              & \quantVal{21.49} & \quantVal{0.712}
              
              & \quantVal{31.09} & \quantVal{0.880}
              & \quantVal{25.07} & \quantVal{0.755}  
              
              & \quantVal{34.04} & \quantVal{0.921}
              & \quantVal{29.66} & \quantVal{0.877}
     
              \\
              
              
      \midrule
      
      AWnet~\cite{cheng2020dual}
              & \multirow{2}{*}{\quantSec{1 HR~/~1 LR}}
              & \quantVal{39.88}  & \quantVal{\second{0.986}}
              & \quantVal{\second{36.63}}  & \quantVal{\second{0.977}}
              & \quantVal{\second{35.51}}  & \quantVal{\second{0.967}}
              & \quantVal{31.31}  & \quantVal{0.922}
              & \quantVal{\second{30.79}}  & \quantVal{0.943}
              & \quantVal{\second{27.32}}  & \quantVal{\second{0.858}}
              
              & \quantVal{\second{32.67}} & \quantVal{\second{0.937}}
              & \quantVal{31.08} & \quantVal{0.914}
              
              & \quantVal{37.13} & \quantVal{0.969} 
              & \quantVal{32.51} & \quantVal{0.937}
              
             
              \\ 
        
    CrossNet~\cite{zheng2018crossnet}
              & 
              & \quantVal{\second{40.85}}  & \quantVal{0.968}
              & \quantVal{36.15}  & \quantVal{\second{0.977}}
              & \quantVal{34.73}  & \quantVal{0.961}
              & \quantVal{\second{32.52}}  & \quantVal{\second{0.932}}
               
              & \quantVal{30.46} & \quantVal{\second{0.958}}
              & \quantVal{27.25} & \quantVal{0.856}
              
              & \quantVal{30.48} & \quantVal{0.869}
              & \quantVal{\second{31.58}} & \quantVal{\second{0.915}}
              
              & \quantVal{\second{37.42}} & \quantVal{\second{0.972}}
              & \quantVal{\second{32.98}} & \quantVal{\second{0.948}}
              
              \\      
              
             
        \midrule
        PASS-Net~(Ours)
              & \multirow{1}{*}{\quantSec{3 HR~/~1 LR}}
              
              & \quantVal{\first{41.72}} & \quantVal{\first{0.989}}
              & \quantVal{\first{38.81}} & \quantVal{\first{0.982}}
              
              & \quantVal{\first{36.40}} & \quantVal{\first{0.967}}
              & \quantVal{\first{33.66}} & \quantVal{\first{0.948}}
              
              & \quantVal{\first{31.21}} & \quantVal{\first{0.951}}
              & \quantVal{\first{29.44}}  & \quantVal{\first{0.931}}
              
              & \quantVal{\first{34.33}} & \quantVal{\first{0.945}}
              & \quantVal{\first{32.27}} & \quantVal{\first{0.923}}
              
              & \quantVal{\first{38.18}} & \quantVal{\first{0.981}}
              & \quantVal{\first{34.33}} & \quantVal{\first{0.956}}
              
              \\
              
        \bottomrule


  \end{tabular}
    % \vspace{-5pt}  
\end{table*}



==> PID253/compare_tables/compare_prediction.tex <==
\begin{table}[t]
  \caption{
     \textbf{Quantitative comparisons on the next frame prediction on the UCF101 and Vimeo-90K test set.}
  }
%   \vspace{-1mm}
  \label{tab:compare_prediction}
  \footnotesize
  \renewcommand{\tabcolsep}{10pt} % adjust horizontal space
  \renewcommand{\arraystretch}{1.2} % adjust vertical space
\newcommand{\quantTit}[1]{\multicolumn{3}{c}{\scriptsize #1}}
    \newcommand{\quantSec}[1]{\scriptsize #1}
    \newcommand{\quantInd}[1]{\scriptsize #1}
    \newcommand{\quantVal}[1]{\scalebox{0.83}[1.0]{$ #1 $}}
    \newcommand{\quantBes}[1]{\scalebox{0.83}[1.0]{$\uline{ #1 }$}}
  \centering
  \begin{tabular}{lcccc}
    \toprule
    
    \multirow{2}{*}[-0.28em]{Method}   
    %  & Runtime 
    % & Parameters 
     &  \multicolumn{2}{c}{UCF101~\cite{soomro2012ucf101}}
      & \multicolumn{2}{c}{Vimeo-90K~\cite{xue2019video}} \\
    
    %  \cmidrule(l{2pt}r{1pt}){2-3}
    % \cmidrule(l{2pt}r{1pt}){4-5} 
    \cmidrule(lr){2-3}
    \cmidrule(lr){4-5}
    
    % % %\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){a-b}
    & \quantSec{PSNR} & \quantSec{SSIM}  & 
    \quantSec{PSNR} & \quantSec{SSIM} \\
    \midrule
        BeyondMSE~\cite{mathieu2015deep}
              & \quantVal{30.01}  & \quantVal{0.897}
              & \quantVal{26.94}  & \quantVal{0.850}         \\
              
        DVF~\cite{liu2017video}
              & \quantVal{30.29}  & \quantVal{0.901}
              & \quantVal{27.55}  & \quantVal{0.866}    \\ % 
              
        CtrlGen~\cite{hao2018controllable}
              & \quantVal{28.13}   & \quantVal{0.864}
              & \quantVal{26.32}   & \quantVal{0.832}  \\
        
        % \midrule
        
        PASS-Net~-~w/o prop
              & \quantVal{\second{30.50}}  &   \quantVal{\second{0.901}}
              & \quantVal{\second{29.71}}    & \quantVal{\second{0.887}}  \\
        PASS-Net (Ours)
              & \quantVal{\first{31.05}}    & \quantVal{\first{0.910}}
              & \quantVal{\first{30.30}}    & \quantVal{\first{0.899}}  \\

        \bottomrule


  \end{tabular}
    \vspace{-10pt}  
\end{table}



==> PID253/images/arch.tex <==
\begin{figure*}[t]
	\footnotesize
    % \scriptsize

	\centering
% 	\renewcommand{\tabcolsep}{1.0pt} % adjust horizontal space
% 	\renewcommand{\arraystretch}{1.0} % adjust vertical space
% 	\begin{tabular}{c}
	\includegraphics[width= 1.0\textwidth]{images/arch.png}
	
% \end{tabular}
%  	\vspace{-5pt}
	\caption{
		\textbf{Illustration of lossy video streaming.} 
		%
		We propose to restore high-resolution (HR) frames at the current time under two streaming patterns.
		%
		First, when current frames are too late to receive before rendering deadline, we proposed to use previously received high-resolution images to predict the future frames.
        %
        Second, when the resolution of the current frames is low (i.e., LR), we propose to use previous high-resolution frames to enhance the current low-quality frames.
	}
%  	\vspace{-10pt}
	\label{fig:arch} 
\end{figure*}



==> PID253/images/flow_propa.tex <==
\begin{figure*}[h]
	\footnotesize
    % \scriptsize

	\centering
% 	\renewcommand{\tabcolsep}{1.0pt} % adjust horizontal space
% 	\renewcommand{\arraystretch}{1.0} % adjust vertical space
% 	\begin{tabular}{c}
	\includegraphics[width= 0.6\textwidth]{images/flow_propa.png}
	
% \end{tabular}
%  	\vspace{-5pt}
	\caption{
		\textbf{Illustration of flow propagation.} 
	}
%  	\vspace{-10pt}
	\label{fig:flow_propa} 
\end{figure*}



==> PID253/images/framework.tex <==
\begin{figure*}[t]
	\footnotesize
    % \scriptsize

	\centering
% 	\renewcommand{\tabcolsep}{1.0pt} % adjust horizontal space
% 	\renewcommand{\arraystretch}{1.0} % adjust vertical space
% 	\begin{tabular}{c}
	\includegraphics[width= 1.0\textwidth]{images/framework.png}
	
% \end{tabular}
%  	\vspace{-5pt}
	\caption{
		\textbf{Architecture of the proposed prediction-assistant video frame super-resolution model.} 
		%
		Given three previously received HR frames $\mathbf{I}_{-2}, \mathbf{I}_{-1},\mathbf{I}_0$, and one current LR frame $\mathbf{I}_t^{\downarrow s}$, where $s$ is the scale factor.
		%
		We first use the three HR frames to predict two optical flows, including the warped flow $\mathbf{\hat{F}}_{0 \rightarrow t}$, and the propagated flow $\mathbf{\tilde{F}}_{0 \rightarrow t}$.
		%
		We also estimate a flow $\mathbf{\bar{F}}_{0 \rightarrow t}$ using HR frame $\mathbf{I}_0$ and the up-scaled current LR frame $\texttt{bic}(\mathbf{I}_t^{\downarrow s})$.
		%
		Then, the three flows are refined by a flow fusion network.
		%
		We then project the fused flow and back-warp the frame $\mathbf{I}_0$ based on the projected flow $\mathbb{F}_{t \rightarrow 0}$.
		%
		Finally, we apply a frame synthesis network to generate the output frame.
		%
		When the current LR frame $\mathbf{I}_t^{\downarrow s}$ is not received before rendering deadline, the proposed model is the same except those green modules.
	}
%  	\vspace{-10pt}
	\label{fig:framework} 
\end{figure*}


==> PID253/images/u-net.tex <==
\begin{figure}[t]
	\footnotesize
    % \scriptsize

	\centering
% 	\renewcommand{\tabcolsep}{1.0pt} % adjust horizontal space
% 	\renewcommand{\arraystretch}{1.0} % adjust vertical space
% 	\begin{tabular}{c}
	\includegraphics[width= 0.475\textwidth]{images/u-net.png}
	
% \end{tabular}
 	\vspace{-5pt}
	\caption{
		\textbf{Architecture of the U-Net used in Flow Fusion module and Frame Synthesis Module.} 
	}
 	\vspace{-5pt}
	\label{fig:u-net} 
\end{figure}



==> PID253/macro.tex <==
% =========================================
% 	Packages
% =========================================
%\usepackage{mathptmx}
\usepackage{xspace}
\usepackage{color}
\usepackage{multirow}
\usepackage{graphics}
\usepackage{adjustbox}
\usepackage{subfigure}
\usepackage{amsmath}
\usepackage{paralist} % compactitem, compactenum
\usepackage{enumitem} % adjust enum margin
\usepackage{booktabs} % Publication quality tables
\usepackage{array}
\usepackage{grffile}
\usepackage{makecell}
\usepackage{diagbox}

% \newcommand\empthDiag[2][]{%
% \diagbox[innerwidth=\widthof{#2},height=\line,#1]{}{}%
% }

\graphicspath{{figures/}}
% \graphicspath{{images/}}

\usepackage[pagebackref=true,breaklinks=true,letterpaper=true,colorlinks,bookmarks=false,citecolor=blue,linkcolor=blue]{hyperref}

% =========================================
% 	Macros
% =========================================
%%% short-hand notations
%\newcommand{\Paragraph}[1]{\paragraph{\textbf{#1}}} % avoid indent for paragraph title
\newcommand{\Paragraph}[1]{{\vspace{-2mm}\flushleft\textbf{#1}}} % avoid indent for
\newcommand{\ul}[1]{\underline{\smash{#1}}}
\newcommand{\tb}[1]{\textbf{#1}}
\newcommand{\mb}[1]{\mathbf{#1}}
\newcommand{\TODO}[1]{{\textbf{\color{red}[TODO: #1]}}}
\newcommand{\n}{\vskip\baselineskip}
\def\ith{i^\textit{th}}

%%% comments
\newcommand {\shenwang}[1]{{\color{red}\textbf{Wang: }#1}\normalfont}
% \newcommand {\shenwang}[1]{{\color{red}\textbf{}#1}\normalfont}
\newcommand {\wenbo}[1]{{\color{blue}\textbf{Wenbo: }#1}\normalfont}
\newcommand {\xiongkuo}[1]{{\color{blue}\textbf{Xiongkuo: }#1}\normalfont}

% \newcommand{\myred}[1]{\textcolor{Mahogany}{\textbf{#1}}}
% \newcommand{\myblue}[1]{\textcolor{blue}{\underline{#1}}}

\newcommand{\myred}[1]{\first{#1}}
\newcommand{\myblue}[1]{\second{#1}}

%%% ignore paragraph
\long\def\ignorethis#1{}

\def\OurTPAMIs{MEMC-Net} 
\def\OursFull{Space-Time Network Pyramid}
\def\OursFullB{Recurrent Space-Time Network Pyramid}
\def\OursHalfBH{Recurrent Network Pyramid}
\def\OursHalfBHSamll{recurrent network pyramid}
\def\OursFullBModule{Inter-Pyramid Recurrent Module}
\def\OursFullBModuleSmall{inter-pyramid recurrent module}
\def\OursFullBModuleSmallR{inter-pyramid Recurrent module}
\def\OursFullBSmall{recurrent space-time network pyramid}
\def\OursFullBSmallR{Recurrent space-time network pyramid}
\def\OursFullSmall{space-time network pyramid}
\def\OursHalfSmall{network pyramid}
\def\OursHalf{Network Pyramid}
\def\Ours{BIN}
\def\OursHalfS{STNP}

\def\SpaAndTime{space and time}
\def\SpaTime{space-time}
\def\figsize{0.08}
\def\Tabarraystretch{1.0}
%\def\OursConvLstmFirst{$\text{PFRN}_{2} \textit{-ConvLSTM}$}
%\def\OursConvLstmThird{$\text{PFRN}_{3} \textit{-ConvLSTM}$}

\def\OursConvLstmFirst{$\text{\Ours}_{2}$}
\def\OursConvLstmSecond{$\text{\Ours}_{3}$}
\def\OursConvLstmThird{$\text{\Ours}_{4} \textit{ -w/o cycle loss}$}
\def\OursConvLstmThirdwithCyc{$\text{\Ours}_{4} \textit{ -w/ cycle loss}$}

\def\OursThirdNewLoss{$\text{\Ours}_{4}$}

% \newcommand{\leftright}[1]{\{ {#1}  \}}

\newcommand{\leftright}[1]{{#1}}

% \def\SpaAndTime{spatial and temporal}

%\def\OursLstmFirst{$\text{PFRN}_{2} \textit{-LSTM}$}
%\def\OursFirst{$\text{PFRN}_{2}$}
%\def\OursThird{$\text{PFRN}_{3}$}

\def\OursLstmFirst{$\text{\Ours}_{2} \textit{ -LSTM}$}
\def\OursConvLstmFirstY{$\text{\Ours}_{2} \textit{ -ConvLSTM}$}
% \def\OursFirst{$\text{PRN}_{2} \textit{ -w/o ConvLSTM} $}
% \def\OursThird{$\text{PRN}_{3} \textit{ -w/o ConvLSTM}$}
\def\OursFirst{$\text{\OursHalfS}_{2}$}
\def\OursSecond{$\text{\OursHalfS}_{3}$}
\def\OursThird{$\text{\OursHalfS}_{4}$}

\def\OursSecondWithoutCyc{$\text{\OursHalfS}_{3} \textit{ -w/o cycle}$}



\def\Input{\mathbf{\hat{I}}_{3}^t}
\def\Hidden{\mathbf{H}^{t}_{3}}
\def\HiddenPrevious{\mathbf{H}_{3}^{t\text{-}1}}
\def\InputGate{i_{3}^{t}}
\def\ForgetGate{f_{3}^t}
\def\OutputGate{o_{3}^t}
\def\Cell{\mathbf{C}_{3}^{t}}
\def\CellPrevious{\mathbf{C}_{3}^{t\text{-}1}}
\def\CellTilde{\mathbf{\tilde{C}}_{3}^{t}}
    

\def\OursFirstNa{$\text{\Ours}_{2} \textit{ -None}$}

\usepackage{tabularx}

%%% color
\definecolor{B1}{RGB}{237,219,201}
\definecolor{MyBlueb}{RGB}{95,169,236}
\definecolor{MyOrange}{RGB}{255,177,98}
\definecolor{MyReda}{RGB}{193,39,45}
\definecolor{gray}{rgb}{0.5,0.5,0.5}
\definecolor{MyBlue}{rgb}{0,0,1.0}
\definecolor{MyYellow}{rgb}{0.9,0.9,0}
\definecolor{MyRed}{rgb}{0.8,0.2,0}
\definecolor{MyGreen}{rgb}{0,0.5,0.0}
\definecolor{MyGray}{rgb}{0.4,0.4,0.4}
\def\newtext#1{\textcolor{blue}{#1}}
\def\torevise#1{\textcolor{red}{#1}}
%\def\modtext#1{#1} % temporary used for submission
\def\red#1{\textcolor{MyRed}{#1}}
\def\blue#1{\textcolor{MyBlue}{#1}}
\def\green#1{\textcolor{MyGreen}{#1}}
\def\yellow#1{\textcolor{MyYellow}{#1}}
\def\myorange#1{\textcolor{MyOrange}{#1}}
\def\myblue#1{\textcolor{MyBlueb}{#1}}
\def\myreda#1{\textcolor{MyReda}{#1}}
\def\mybone#1{\textcolor{B1}{#1}}

\def\first#1{\red{\textbf{#1}}}
\def\second#1{\blue{\underline{#1}}}
\def\fbone#1{\myorange{\textbf{#1}}}
\def\fbtwo#1{\myblue{\textbf{#1}}}
\def\reda#1{\myreda{\textbf{#1}}}
\def\bone#1{\mybone{\textbf{#1}}}


\def\firstonly#1{\textbf{#1}}

%%% adjust margin
\newlength\paramargin
\newlength\figmargin
\newlength\secmargin

\setlength{\paramargin}{-1.0mm}
\setlength{\figmargin}{-1.5mm}
\setlength{\secmargin}{-2.5mm}

%% table control
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

%% Latin abbreviations 
\def\ie{i.e.,~}
\def\eg{e.g.,~}
\def\etc{etc}
\def\cf{cf.~}
\def\viz{viz.~}
\def\vs{vs.~}
\def\etal{et~al.\xspace}
\def\Naive{Na\"{\i}ve~}
\def\naive{na\"{\i}ve~}

% symbols using in math
%\DeclareMathOperator*{\argmin}{\arg\!\min}
%\DeclareMathOperator*{\argmax}{\arg\!\max}

\setlength{\fboxsep}{0pt}
\def\padg{{\color{white}g}}

\newcommand{\jbox}[2]{
  \fbox{%
  	\begin{minipage}{#1}%
  		\hfill\vspace{#2}%
  	\end{minipage}%
  }}

\newcommand{\jblock}[2]{%
	\begin{minipage}[t]{#1}\vspace{0cm}\centering%
	#2%
	\end{minipage}%
	}

%% reference macro
% \newcommand{\secref}[1]{Section~\ref{sec:#1}}
% \newcommand{\figref}[1]{Figure~\ref{fig:#1}}
% \newcommand{\tabref}[1]{Table~\ref{tab:#1}}
% \newcommand{\eqnref}[1]{\eqref{eq:#1}}
% \newcommand{\thmref}[1]{Theorem~\ref{#1}}
% \newcommand{\prgref}[1]{Program~\ref{#1}}
% \newcommand{\algref}[1]{Algorithm~\ref{#1}}
% \newcommand{\clmref}[1]{Claim~\ref{#1}}
% \newcommand{\lemref}[1]{Lemma~\ref{#1}}
% \newcommand{\ptyref}[1]{Property~\ref{#1}}

\newcommand{\secref}[1]{Section~\ref{#1}}
\newcommand{\figref}[1]{Figure~\ref{#1}}
\newcommand{\tabref}[1]{Table~\ref{#1}}
\newcommand{\eqnref}[1]{Equation~\eqref{#1}}
\newcommand{\thmref}[1]{Theorem~\ref{#1}}
\newcommand{\prgref}[1]{Program~\ref{#1}}
\newcommand{\algref}[1]{Algorithm~\ref{#1}}
\newcommand{\clmref}[1]{Claim~\ref{#1}}
\newcommand{\lemref}[1]{Lemma~\ref{#1}}
\newcommand{\ptyref}[1]{Property~\ref{#1}}



\newcommand{\dummyfig}[1]{
	\centering
	\fbox{
		\begin{minipage}[c][0.33\textheight][c]{0.5\textwidth}
			\centering{#1}
		\end{minipage}
	}
}


\newcommand{\veryshortarrow}[1][3pt]{\mathrel{%
		\hbox{\rule[\dimexpr\fontdimen22\textfont2-.2pt\relax]{#1}{.4pt}}%
		\mkern-5mu\hbox{\usefont{U}{lasy}{m}{n}\symbol{41}}}}

\makeatletter

\setbox0\hbox{$\xdef\scriptratio{\strip@pt\dimexpr
		\numexpr(\sf@size*65536)/\f@size sp}$}

\newcommand{\scriptveryshortarrow}[1][5pt]{{%
		\hbox{\rule[\scriptratio\dimexpr\fontdimen22\textfont2-.2pt\relax]
			{\scriptratio\dimexpr#1\relax}{\scriptratio\dimexpr.4pt\relax}}%
		\mkern-5mu\hbox{\let\f@size\sf@size\usefont{U}{lasy}{m}{n}\symbol{41}}}}

\makeatother

